(Re)configuration based on model generation

Reconfiguration is an important activity for companies selling configurable products or services which have a long life time. However, identification of a set of required changes in a legacy configuration is a hard problem, since even small changes in the requirements might imply significant modifications. In this paper we show a solution based on answer set programming, which is a logic-based knowledge representation formalism well suited for a compact description of (re)configuration problems. Its applicability is demonstrated on simple abstractions of several real-world scenarios. The evaluation of our solution on a set of benchmark instances derived from commercial (re)configuration problems shows its practical applicability.

==> eptcsdata.tex <==
\providecommand{\firstpage}{26}
\providecommand{\publicationstatus}{C. Drescher, I. Lynce and R. Treinen (eds.):\\ Workshop on Logics for Component Configuration (LoCoCo 2011)\\
EPTCS 65, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.65.3}{10.4204/EPTCS.65.3}}
\pdfoutput=1

